All In Good Time: Causality-Aware Framework for LLM-Based Simultaneous Speech-to-Speech Translation

Large Language Models (LLMs) have shown strong performance in low-resource offline translation; however, extending them to simultaneous speech-to-speech translation (Simul-S2ST) remains challenging due to the scarcity of causally aligned training data with high cross-lingual speaker fidelity. In addition, existing approaches rely on fixed translation policy or confidence heuristics, leading to suboptimal quality and higher latency. We propose a causality-aware Simul-S2ST framework with a novel data pipeline that generates high-fidelity, causally aligned segments with improved voice transfer. The framework introduces (i) a factorized S2ST architecture (FAST), (ii) a causality-aware adaptive policy (CAP), and (iii) causality-aware latency metric. Experiments on CVSS Spanish, German, and French show that FAST-CAP consistently improves the quality-latency trade-off, achieving up to +1.2 BLEU and a 26% relative latency reduction over a fixed policy. Despite using substantially less training data than existing systems, FAST-CAP achieves state-of-the-art results in speech translation quality and speaker fidelity while yielding up to a 38.8% relative reduction in latency.

==> tables/speech_quality.tex <==
\setlength{\tabcolsep}{2pt}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l c c c c c c}
\toprule
 & \multicolumn{2}{c}{\textbf{Es--En}} & \multicolumn{2}{c} {\textbf{De--En}} & \multicolumn{2}{c}{\textbf{Fr--En}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \textbf{System}
 & \textbf{UTMOS} & \textbf{Spk-Sim} & \textbf{UTMOS} & \textbf{Spk-Sim} & \textbf{UTMOS} & \textbf{Spk-Sim} \\
\midrule
Multilingual (offline)     & 2.3 & 0.30 & 2.4 & 0.26 & 2.3 & 0.27 \\
\midrule
Monolingual (Simul.)   & 1.8 & 0.30 & 1.3 & 0.21 & 1.9 & 0.26 \\
Multilingual (Simul.)  & 1.8 & 0.30 & \textbf{2.0} & \textbf{0.26} & 1.9 & 0.26 \\
\bottomrule
\end{tabular}
}
